No learning rates needed: Introducing SALSA -- Stable Armijo Line Search Adaptation

In recent studies, line search methods have been demonstrated to significantly enhance the performance of conventional stochastic gradient descent techniques across various datasets and architectures, while making an otherwise critical choice of learning rate schedule superfluous. In this paper, we identify problems of current state-of-the-art of line search methods, propose enhancements, and rigorously assess their effectiveness. Furthermore, we evaluate these methods on orders of magnitude larger datasets and more complex data domains than previously done. More specifically, we enhance the Armijo line search method by speeding up its computation and incorporating a momentum term into the Armijo criterion, making it better suited for stochastic mini-batching. Our optimization approach outperforms both the previous Armijo implementation and a tuned learning rate schedule for the Adam and SGD optimizers. Our evaluation covers a diverse range of architectures, such as Transformers, CNNs, and MLPs, as well as data domains, including NLP and image data. Our work is publicly available as a Python package, which provides a simple Pytorch optimizer.

==> ablation.tex <==

In this section we will take a short look at which parts of our PLASLS approach have the most impact on performance, as well as different options for multiple elements of the described algorithm which we tested, but did not go into detail in the other sections.

\subsection{Batch size}

During our experiments we noticed that the batch size had a large influence on the stability of the training. In this section we compare different batch sizes.

\begin{figure}
\includegraphics[width = 0.45\textwidth]{figures/lossSST2batchsize.png}
\caption{Loss on the sst2small dataset for different batch size options for PLASLS. Standard error is visualized around each line. The X-Axis denotes the number of samples processed.}
\label{fig:batchsize}
\end{figure}

In Figure \ref{fig:batchsize}, we see that PLASLS performance improves for larger batch sizes during training. Furthermore, the loss curves get a lot smoother with higher batch sizes. During our experiments we choose a batch size of 32 as it was the highest supported batch size on our available hardware.

\subsection{Split Options}
Several possibilities to split a Transformer based network exist. In this section we look at a split by:
\begin{itemize}
    \item layer 
    \item query, key and value
\end{itemize}
We tried splitting the network in 1,4,7,10 components as well as by query,key and value (QKV). If we split the network in one component, ADAMSLS is equivalent to PLASLS. The loss curves for different layer configurations can be seen in Figure \ref{fig:layer}.
More layers result in gradually better performance for the SST2small dataset.
Splitting by QKV does not seem to improve performance.
\begin{figure}
\includegraphics[width = 0.45\textwidth]{figures/sst2Numsplit.png}
\caption{Loss on the SST2small dataset for different split options for PLASLS and ADAMSLS as reference. Standard error is visualized around each line.}
\label{fig:layer}
\end{figure}








\iffalse
\subsection{Update rule}

In Section \ref{sec:methods}, we described a simple rule to determine the update order of the subunits used in PLASLS. We designed a more complex update rule we call "magnitude based" to prioritize updating sections of the network which have a larger impact on the change of loss. 

The magnitude based update rule works as follows:

First we compute the impact upon the loss a subnetwork $S_k$ has ,we call this $\Delta L(S_k)$:
\begin{equation}
  \Delta L(S_k) =  f_{ik}(w_k) - f_{ik}(w_k - n_k \nabla f_{ik}(w_k))
\end{equation}
$w_k$ references the weights of the subnetwork $S_k$.
To save on compute and obtain a more stable approximation of this value, we use the exponential moving average of $\Delta L_{i+1}(S_k) = \Delta L(S_k)*\omega + (1-\omega)* \Delta L_i(S_k)$. With $\omega = 0.9$
When this change of loss is large the loss of the whole network is susceptible to updates to the weights of this subnetwork in particular. So it is sensible to update the step size of subnetworks with large $\Delta L(S_k)$ more often.
Additionally, we want to assign a higher probability $P(S_k)$ to a subnetwork to get updated, the longer it has not been updated.
\begin{equation}
  P(S_k) = \lambda 2^{T_k} + \frac{\Delta L(S_k)}{\sum_k \Delta L(S_k)}
\end{equation}
$T_k$ is the number of iterations since this subnetwork has last been updated. $\lambda$ is a weighting factor.
To obtain the final probability $P(S_k)$  we normalize $P(S_k)$.
\begin{equation}
  P_f(S_k) = \frac{P(S_k)}{\sum_k P(S_k)}
\end{equation}

\begin{figure}
\includegraphics[width = 0.45\textwidth]{figures/sst2impact.png}
\caption{Loss on the sst2small dataset for different update rule options for PLASLS. Standard error is visualized around each line.}
\label{fig:impactMag}
\end{figure}

In Fig. \ref{fig:impactMag} we see the results of our experiments for the update rule, a magnitude based update order seems to make the results have a higher variance, but small to no improvements can be detected.
\fi


==> limitations.tex <==

In this section we will go into various Limitations of our work as well as work in progress.

\begin{itemize}
    \item one extra forward pass per step required.
    \item needs to encapsulate the forward pass -> not quite as easy to use as a normal optimizer
    %\item for multi-gpu training even more extra code is needed
    \item gpt-2 pre-training did result in very low learning rates.
    %\item gradient scaling, which used for training with float16 precision and large architectures does not work with our current optimizer
    %\item did not work well for graph neural networks (only 1 tested)
  %  \item with c=0.5 convergence did happen but in some cases sSLS did introduce an initial low learning rate phase that slowed down convergence.
\end{itemize}

==> theorem.tex <==
We extend the convergence Theorem of \cite{armijo66a} for the full batch setting and the SaLSa criterion.
We additionally require that every found learning rate yields an improved loss.
In practice, this additional condition does not affect the optimization significantly.
\begin{theorem}[Convergence Theorem]
    Let $f \equiv f_k$.
    For $w_0 \in \mathbb{R}^d$ let $S(w_0) := \{w \mid f(w) \leq f(w_0)\}$ and assume that $f(w^*) := \inf_{w \in \mathbb{R}^d} f(w)$ exists for a unique point $w^* \in \mathbb{R}^d$ with $\nabla f(w) = 0$ for $w \in S(w_0)$ if and only if $w = w^*$.
    Any sequence $\{w_{k}\}_{k=1}^\infty$ found by the SaLSa criterion with $f(w_k) - f(w_k + \eta_k d_k) \geq 0$ and $c < 1$ converges to $w^*$.
\end{theorem}

\begin{proof}
    Given the condition $f(w_i) - f(w_i + \eta_i d_i) \geq 0$ ensures that $\{f(w_i)\}_{i=1}^k$ is non-increasing and thus any infinite sequence will converge to $f(w^*)$, given the assumptions.
    It thus remains to show, that in every step such a step size $\eta_i$ can be found.
    By definition, we have that
    \begin{align*}
        h_k &= \beta_3 h_{k-1} + (1-\beta_3) \left[f(w_k) - f(w_k + \eta_k d_k)\right]
        \\
        &\geq \beta_3 c \eta_{k-1} s_{k-1} + (1-\beta_3) \left[f(w_k) - f(w_k + \eta_k d_k)\right].
    \end{align*}
    It remains to show that there exists a learning rate $\eta_k\leq\eta_{k-1}$, such that $f(w_k) - f(w_k + \eta_k d_k) \geq c \eta_k \Vert \nabla f(w_k)\Vert^2$. 
    Then,
    \begin{align*}
        \beta_3 c \eta_{k-1} s_{k-1} + (1-\beta_3) \left[f(w_k) - f(w_k + \eta_k d_k)\right] &\geq c \eta_{k}\left[\beta_3 s_{k-1} + (1-\beta_3) \Vert \nabla f(w_k)\Vert^2\right]
        \\
        &= c \eta_{k} s_{k}.
    \end{align*}
    We prove the existence of $\eta_k$ by contradiction, i.e. we assume that such a $\eta_k$ does not exist and thus $f(w_k) - f(w_k + \eta_k d_k) < c \eta_k \Vert \nabla f(w_k)\Vert^2$ for $\eta_k \leq \eta_{k-1}$. Then, using the Taylor expansion for $f$ around $f(w_k)$ yields 
    \begin{align*}
         f(w_k) - f(w_k + \eta_k d_k) = -\eta_k d_k \nabla f (w_k) - o(\eta_k).
    \end{align*}
    For $\eta_k \leq \eta_{k-1}$ it follows by assumption
    \begin{align*}
        c \eta_k \Vert \nabla f(w_k)\Vert^2 > -\eta_k d_k \nabla f (w_k) - o(\eta_k).
    \end{align*}
    Dividing both sides by $\eta_k$ and taking the limit for $\eta_k \to 0$ yields
    \begin{align*}
         c \Vert \nabla f(w_k)\Vert^2 > -d_k \nabla f (w_k),
    \end{align*}
    and thus with $d_k = - \nabla f(w_k)$ it follows $c > 1$, which is a contradiction.
\end{proof}
